Language-Guided Image Tokenization for Generation

Image tokenization, the process of transforming raw image pixels into a compact low-dimensional latent representation, has proven crucial for scalable and efficient image generation. However, mainstream image tokenization methods generally have limited compression rates, making high-resolution image generation computationally expensive. To address this challenge, we propose to leverage language for efficient image tokenization, and we call our method Text-Conditioned Image Tokenization (TexTok). TexTok is a simple yet effective tokenization framework that leverages language to provide a compact, high-level semantic representation. By conditioning the tokenization process on descriptive text captions, TexTok simplifies semantic learning, allowing more learning capacity and token space to be allocated to capture fine-grained visual details, leading to enhanced reconstruction quality and higher compression rates. Compared to the conventional tokenizer without text conditioning, TexTok achieves average reconstruction FID improvements of 29.2% and 48.1% on ImageNet-256 and -512 benchmarks respectively, across varying numbers of tokens. These tokenization improvements consistently translate to 16.3% and 34.3% average improvements in generation FID. By simply replacing the tokenizer in Diffusion Transformer (DiT) with TexTok, our system can achieve a 93.5x inference speedup while still outperforming the original DiT using only 32 tokens on ImageNet-512. TexTok with a vanilla DiT generator achieves state-of-the-art FID scores of 1.46 and 1.62 on ImageNet-256 and -512 respectively. Furthermore, we demonstrate TexTok's superiority on the text-to-image generation task, effectively utilizing the off-the-shelf text captions in tokenization. Project page is at: https://kaiwenzha.github.io/textok/.

==> tables/tab-t2i.tex <==
\begin{table}[t]
    \begin{center}
    \footnotesize
    \begin{tabular}{lccc}
    \midrule
    tokenizer & generator & FID$\downarrow$   & CLIP Score$\uparrow$ \\
    \midrule
     Baseline-32 \footnotesize{(w/o text)} & \multirow{2}{*}{DiT-XL-T2I} & 5.09 & 28.08 \\
    \textbf{TexTok-32 \footnotesize{(w/ text)}} & & \textbf{4.36} & \textbf{28.73} \\
    \midrule
     Baseline-64 \footnotesize{(w/o text)} & \multirow{2}{*}{DiT-XL-T2I} & 3.74 & 28.49 \\
    \textbf{TexTok-64 \footnotesize{(w/ text)}} & & \textbf{3.34} & \textbf{28.92} \\
    \midrule
    Baseline-128 \footnotesize{(w/o text)} & \multirow{2}{*}{DiT-XL-T2I} & 3.01 & 28.95 \\
    \textbf{TexTok-128 \footnotesize{(w/ text)}} & & \textbf{2.82} & \textbf{29.23} \\
    \bottomrule
    \end{tabular}
    \end{center}
    \vspace{-4mm}
    \caption{\footnotesize \textbf{Text-to-image generation performance of TexTok comparing with \wotext{}}  on ImageNet 256$\times$256.
    TexTok achieves better FID and CLIP scores on all 32/64/128-token settings, demonstrating that TexTok produces image tokens that improve text-to-image generation results, \textit{using the exactly same image generation setups}. Classifier-free guidance is applied.}  %
    \label{tab:t2i}
\end{table}
